CINM (Cinnamon): A Compilation Infrastructure for Heterogeneous Compute In-Memory and Compute Near-Memory Paradigms

The rise of data-intensive applications exposed the limitations of conventional processor-centric von-Neumann architectures that struggle to meet the off-chip memory bandwidth demand. Therefore, recent innovations in computer architecture advocate compute-in-memory (CIM) and compute-near-memory (CNM), non-von- Neumann paradigms achieving orders-of-magnitude improvements in performance and energy consumption. Despite significant technological breakthroughs in the last few years, the programmability of these systems is still a serious challenge. Their programming models are too low-level and specific to particular system implementations. Since such future architectures are predicted to be highly heterogenous, developing novel compiler abstractions and frameworks become necessary. To this end, we present CINM (Cinnamon), a first end-to-end compilation flow that leverages the hierarchal abstractions to generalize over different CIM and CNM devices and enable device-agnostic and device-aware optimizations. Cinnamon progressively lowers input programs and performs optimizations at each level in the lowering pipeline. To show its efficacy, we evaluate CINM on a set of benchmarks for the well-known UPMEM CNM system and the memristors-based CIM accelerators. We show that Cinnamon, supporting multiple hardware targets, generates high-performance code comparable to or better than state-of-the-art implementations.

==> contents/base2.tex <==
% Summary.
We designed an \gls{ssa} \gls{ir} called \projectsc to address the programmability challenges for arbitrary-precision arithmetic.
We implemented this \gls{ir} as a set of \MLIR dialects.
The \projecttt dialect is a new medium-level abstraction layer for target-agnostic \gls{ir} producers, such as linear algebra front-ends.
One of our explicit design goals is to replace \texttt{arith} in all contexts, thus avoiding signless integers and unwanted \gls{ub} above the code-selection level.

\subsection{Type hierarchy}

% What is the type hierarchy of base2?
\projectsc is designed to be minimal but complete with respect to the most common binary number formats.
To simplify implementation and extensibility, the requirements placed on its member types are layered.
To that extent, \projectsc defines an internal hierarchy of types, as depicted in \cref{fig:type_hierarchy}.
In summary:
\begin{itemize}
    \item \textbf{Bit sequence types} are represented by bit sequences of a fixed length \BwidthT[B].
    \item \textbf{Interpretable types} are bit sequence types with an associated interpretation function \InterpT[P], i.e., a (reversible) function that maps bit sequences to points.
    \item \textbf{Number types} are interpretable types with an associated rounding function \RoundTR[N], i.e., a function that maps rational numbers to points under a given rounding mode \(R\).
    \item \textbf{Fixed-point types} are number types represented by canonical integers with an associated fixed exponent.
    \item \textbf{Floating-point types} are number types decomposable into an integer significand and exponent of base \(2\).
\end{itemize}

\begin{figure}[htbp]
    \centering
    % \begin{tikzpicture}[yscale=0.8]
    %     \tikzset{type/.style = {shape=rectangle,draw,minimum size=1.5em}}
    %     \tikzset{specialization/.style = {->,>=Triangle}}

    %     \node[type] (B) at (0,3) {Bit sequence type \Type[B]};
    %     \node[type] (P) at (0,2) {Interpretable type \Type[P]};
    %     \node[type] (N) at (0,1) {Number type \Type[N]};
    %     \node[type] (F) at (-2,0) {Fixed-point type \Type[F]};
    %     \node[type] (R) at (2,0) {Floating-point type \Type[R]};
    %     \node[type] (I) at (-2,-1) {Integer type \Type[I]};

    %     \draw[specialization] (I) to (F);
    %     \draw[specialization] (R) to (N);
    %     \draw[specialization] (F) to (N);
    %     \draw[specialization] (N) to (P);
    %     \draw[specialization] (P) to (B);

    %     \tikzset{annot/.style = {shape=rectangle}}

    %     \node[annot] at (4.2,3) {\BwidthT[B]};
    %     \node[annot] at (4.2,2) {\InterpT[P]};
    %     \node[annot] at (4.2,1) {\RoundTR[N]};
    %     \node[annot] at (4.2,0) {\(z, E\)};
    % \end{tikzpicture}
    \includegraphics{figures/type-hierarchy.pdf}
    \caption{The \projectsc type hierarchy.}
    \label{fig:type_hierarchy}
\end{figure}

% What do the requirements provide?
These requirements are sufficient to generalize the common operations to all number types.
This allows for type- and thus target-independent contracts to be established by the specification.
From these requirements, we derive additional tools such as the subtype relation and the type promotion operator (least common supertype).

% Pre-defined types.
The scope of \projectsc is limited to fixed-point and floating-point binary rationals.
While the canonical cyclic integer representation fully defines every allowed fixed-point format, the same is not true for floating-point encodings.
Fixed-point and integer types are totally specified by \projectsc, whereas floating-point formats may exhibit \impldef behavior.

\subsection{Operation definitions}

% How are the operations defined?
\projectsc provides the common, closed arithmetic operations of addition, subtraction, multiplication, division and remainder.
These operations rely on an inherent rounding mode, which constrains the result.
We define all of them by applying the type-specific rounding function to the exact mathematical result, which is obtained through interpretation, e.g.
\begin{equation*}
    \texttt{add}(a, b, R) = \RoundTR[N]\left(\InterpT[N](a) + \InterpT[N](b)\right)
\end{equation*}

% What about the remainder?
As another example, the remainder operation disambiguates the ``modulo'' operator using a rounding mode \(R\) via
\begin{equation*}
    \texttt{rem}(a, b, R) = \InterpT[N](a) - \InterpT[N](b)\texttt{div}(a, b, R)
\end{equation*}

% What about bit manipulation?
To remain independent of the encoding, \projectsc does not allow bit manipulation.
Some common bit-centric operations can still be expressed in a compatible and portable manner.
For example, the (arithmetic) bit shifting operations with \(z \in \mathbb{Z}\) and \(k,n \in \mathbb{N}\) are given by
\begin{align*}
    \texttt{shl}(z, k) &\equiv z \cdot 2^k \mod 2^n \\
    \texttt{shr}(z, k) &= \lfloor z \cdot 2^{-k} \rfloor
\end{align*}

% What about overflow?
Overflow and underflow in \projectsc are covered by the rounding modes.
Depending on the requested rounding, the constraints from \cref{fig:rounding_constraints} force a certain saturation behavior as shown in \cref{fig:saturation}.

\begin{figure}[htbp]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}[h]{1.0\columnwidth}
        \centering
        \begin{tabular}{rccr}
            \toprule
            \bfseries Mode & \bfseries Underflow & \bfseries Overflow \\ \midrule
            none           & \multicolumn{2}{c}{\impldef} \\
            exact          & \Poison    & \Poison \\ \midrule
            nearest        & \(\min Y\) & \(\max Y\) \\
            down           & \impldef   & \(\max Y\) \\
            up             & \(\min Y\) & \impldef \\
            towards zero   & \(\min Y\) & \(\max Y\) \\
            away from zero & \multicolumn{2}{c}{\impldef} \\
            converge       & \multicolumn{2}{c}{\impldef} \\ \bottomrule
        \end{tabular}
        \caption{Saturation on overflow and underflow.}
        \label{fig:saturation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{1.0\columnwidth}
        \centering
        \begin{tabular}{rcc} \toprule
            \bfseries Mode & \bfseries \(\epsilon_R(z, n)\) \\ \midrule
            none           & \impldef \\
            exact          & --- \\ \midrule
            nearest        & \(2^{-n-1} - \begin{cases}1 & z < 0 \\ 0 & z \ge 0\end{cases}\) \\
            down           & \(0\) \\
            up             & \(2^{-n} - 1\) \\
            towards zero   & \(z \ge 0: \epsilon_\text{down}(z, n)\), \(z < 0: \epsilon_\text{up}(z, n)\) \\
            away from zero & \(z \ge 0: \epsilon_\text{up}(z, n)\), \(z < 0: \epsilon_\text{down}(z, n)\) \\
            converge       & \impldef \\ \bottomrule
        \end{tabular}
        \caption{Rounding bias for fractional rounding.}
        \label{fig:rounding_bias}
    \end{subfigure}
    \caption{Implementation of the rounding modes.}
    \label{fig:rounding_impl}
\end{figure}

% How does this help?
Another aspect of \projectsc is the ability to bootstrap rounding, i.e., implement the rounding modes using exact \projectsc operations.
This is important as not every platform will implement every rounding mode.
For integer saturation, this is trivial.
For fractional rounding, we can make use of previous results.
Let \(z \in \mathbb{Z}\) and \(n \in \mathbb{N}\), it follows that
\begin{align*}
    \RoundTR\left(z \cdot 2^{-n}\right) &= \texttt{div}\left(z^\prime, 2^n, \text{down}\right) \\
    &= \texttt{shr}\left(\texttt{add}\left(z, \epsilon_R(z, n), R\right), n\right)
\end{align*}
where \(\epsilon_R\) is the rounding bias function (cf. \cref{fig:rounding_bias}).

% \subsubsection{Archetype-specific operations}

% % What are the archetype-specific operators?
% We define additional archetype-specific operators based on an expectation of implementation complexity.
% For integer types, we provide the cyclic group integer operations.
% For the fixed-point types, we provide operations that infer the smallest result type that always fits the result value, thus providing guaranteed-exact operations.
% For floating-point types, we intend to provide a common environment of operations that allow unification of fixed-point and floating-point code generation.

% % Why do we need them?
% The ultimate goal is to be able to bootstrap not only fixed-point, but also floating-point operations from within \projectsc.
% \projectsc aims to specify all operations in terms of cyclic integers, but a back-end may choose to exit lowering on a higher level.
% In the meantime, it is desirable to have these high-level operations to be able to map to existing implementations and perform better target code selection.

\subsection{MLIR implementation}

% Summary.
Our \MLIR implementation \texttt{\projectname-mlir}\footnote{\url{https://github.com/KFAFSP/base2-mlir}} is the reference implementation of the \projectsc specification\footnote{\url{https://github.com/KFAFSP/base2-spec}}.
It provides target-agnostic front-ends with contracts for fixed-point and floating-point arithmetic on parametric types.
While fixed-point types are covered in their entirety, the \MLIR implementation is extensible via interfaces to add further formats, especially for floating-point.
The current implementation is incomplete with respect to our unification goals for a common floating-point environment.

\subsubsection{Contracts}

% Contracts.
The new \projecttt dialect is the highest level of abstraction provided by our implementation, and is intended to completely replace \texttt{arith}.
It depends on cyclic integers, which are modeled by the new \texttt{cyclic} dialect.
Bitwise operations are provided by the new \texttt{bit} dialect.
Undefined behavior is modeled using the new \texttt{ub} dialect, which we hope will be provided by the \MLIR core in the future.
All new dialects together with \texttt{index} combine to form a lowering path to \texttt{llvm} (see \cref{fig:base2_mlir_lowering}).
The \gls{ir} elements offered by the new dialects are listed in \cref{tab:base2_mlir_elements}.
%The contract each dialect offers in that scenario is summarized in \cref{tab:dialect_contracts}.
The contract each dialect offers in that scenario is summarized in \cref{fig:contracts}.

% \begin{table}[H]
    % \begin{tabularx}{\textwidth}{>{\bfseries\ttfamily}rX}
    %     \multicolumn{2}{c}{Existing dialects} \\
    %     arith  & The target supports signless integers of arbitrary bit width, and some set of binary floating-point types. They participate in arithmetic with undefined overflow and rounding. \\
    %     index  & The target has an integer type suitable for address computation. Its values are ordered and support arithmetic. Overflow is undefined. \\ \midrule
    %     \multicolumn{2}{c}{\texttt{\projectname-mlir} dialects} \\
    %     bit    & The target supports manipulation of ordered bit sequences. \\
    %     cyclic & The target supports parametric unsigned and signed cyclic integers. \\
    %     \projectname  & The target supports fixed-point and some floating-point arithmetic. \\
    % \end{tabularx}
%     \caption{Dialect contracts in \texttt{\projectname-mlir}.}
%     \label{tab:dialect_contracts}
% \end{table}

\begin{figure}[htbp]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}[h]{1.0\columnwidth}
        \begin{tabular}{>{\bfseries\ttfamily}p{0.1\columnwidth}p{0.85\columnwidth}}
            \multicolumn{2}{c}{Existing dialects} \\
            arith  & Signless integer types of arbitrary bit width. Some binary floating-point types. Arithmetic with underdefined overflow and rounding. \\
            index  & An integer type suitable for address computation. Its values are ordered and support arithmetic. Overflow is explicitly undefined. \\ \midrule
            \multicolumn{2}{c}{\texttt{\projectname-mlir} dialects} \\
            bit    & Manipulation of ordered bit sequences. \\
            cyclic & Parametric unsigned and signed cyclic integers. \\
            \projectname  & Parametric fixed-point and floating-point arithmetic. \\
        \end{tabular}
        \caption{Dialect contracts.}
        \label{fig:contracts}
    \end{subfigure}
    \begin{subfigure}[h]{1.0\columnwidth}
        \centering
        \footnotesize
        \begin{tabular}{>{\ttfamily}r>{\ttfamily}l}
            ub.             & \#poison, poison, freeze \\ \midrule
            bit.            & \#bits, \#dense\_bits, constant, cast, cmp, select \\
                            & and, or, xor, shl, shr, count, clz, ctz \\ \midrule
            cyclic.         & constant, trunc, ext, cmp, min, max, shl, shr \\
                            & add, sub, mul, div, rem \\
            cyclic.checked. & trunc, shl, add, sub, mul, div \\ \midrule
            \projectname.   & !fixed, !ieee754, cast, cmp, min, max,
                              add \\
                            & sub, mul, div, rem \\
            \projectname.fixed. & add, sub, mul, div, rem \\
            \textcolor{gray}{\projectname.float.} & \textcolor{gray}{ilogbn, scalbn} \\
        \end{tabular}
        \caption{Attributes, types and operations in \texttt{\projectname-mlir}. Incomplete features are in \textcolor{gray}{gray}.}
        \label{tab:base2_mlir_elements}
    \end{subfigure}
    \begin{subfigure}[h]{1.0\columnwidth}
        \centering
        % \begin{tikzpicture}[scale=0.9]
        %     \tikzset{dialect/.style = {shape=rectangle,draw,minimum size=1.5em}}
        %     \tikzset{lowering/.style = {->,>=Triangle}}

        %     \node[dialect] (fe) at (0,4) {front-end};
        %     \node[dialect,fill=gray] (arith) at (-1.5,3) {\texttt{arith}};
        %     \node[dialect] (base2) at (1.5,3) {\projecttt};
        %     \node[dialect] (cyclic) at (0.5,2) {\texttt{cyclic}};
        %     \node[dialect] (bit) at (2,1) {\texttt{bit}};
        %     \node[dialect] (ub) at (1,0) {\texttt{ub}};
        %     \node[dialect,fill=gray] (index) at (-0,1) {\texttt{index}};
        %     \node[dialect,fill=gray] (llvm) at (-0.5,0) {\texttt{llvm}};

        %     \draw[lowering,color=gray] (fe) to (arith);
        %     \draw[lowering,color=gray] (arith) to (llvm);
        %     \draw[lowering,color=gray] (index) to (llvm);
        %     \draw[lowering] (fe) to (base2);
        %     \draw[lowering] (base2) to (cyclic);
        %     \draw[lowering] (base2) to (bit);
        %     %\draw[lowering] (base2) to (ub);
        %     \draw[lowering] (cyclic) to (index);
        %     \draw[lowering] (cyclic) to (bit);
        %     %\draw[lowering] (cyclic) to (ub);
        %     \draw[lowering] (bit) to (llvm);
        %     %\draw[lowering] (bit) to (ub);
        % \end{tikzpicture}
        \includegraphics{figures/dialect-stack.pdf}
        \caption{Dialect lowerings in \texttt{\projectname-mlir}. \MLIR core features in \textcolor{gray}{gray}.}
        \label{fig:base2_mlir_lowering}
    \end{subfigure}
    \caption{Breakdown of the \texttt{\projectname-mlir} \MLIR project.}
\end{figure}

\subsubsection{Interfaces}

% Interfaces.
\texttt{\projectname-mlir} is designed for extensibility and reusability.
The implementation relies heavily on \MLIR interfaces and type \& attribute specializations.
This greatly reduces the effort required to add compliant types, even when they are outside the user's control.
For example, the \texttt{FixedPointSemantics} and \texttt{IEEE754Semantics} interfaces seamlessly integrate the built-in types into \texttt{\projectname-mlir}.
Support for handling scalar and container constants of bit sequence types is provided by our \texttt{BitSequenceAttr} and \texttt{DenseBitSequencesAttr} of the \texttt{bit} dialect.
This trivializes the implementation of constant folding that would otherwise be hard to implement for new binary encodings.

\subsubsection{End-to-end usage}

% Intended user proficiency.
For CPU targets, \texttt{\projectname-mlir} is directed at typical users which expect a reasonably efficient and functional lowering pipeline to \texttt{llvm}.
For reconfigurable targets, \texttt{\projectname-mlir} is directed at advanced users that are in posession of either vendor target dialects or pluggable \gls{hls}.
An end-to-end flow requires exiting the \projecttt lowering flow at an interoperable level, for example via \LLVMIR or CIRCT \gls{hls}.

% End-to-end using Bambu.
As users of Bambu HLS~\cite{Ferrandi2021}, we exit at the \texttt{llvm} level, lowering fixed-point entirely, and implementing \texttt{!\projectname.ieee754} via \texttt{libsoftfloat} calls.
We achieve this using a trivial, new \texttt{softfloat} dialect, mapping library operations \(1:1\), which \projecttt can be trivially lowered to, and is in turn trivially lowered to \texttt{func} and thus \texttt{llvm}.


==> contents/overview.tex <==
\section{Motivation and overview}
\label{sec:overview}
\jc{Maybe a more descriptive title: 
``The need for CIM and CNM abstractions''?}
This section motivates
\jc{The prev section also started with ``this section..''. I would suggest using a language that sounds more fluent that implicitly explains the reason for ``this section'' while connecting to the previous. Quick example just to make my point: 
``The aforementioned explosion of technologies and architectures have led to fragmented toolchains and device-specific low-level programming APIs. 
This imposes a high entry barrier for programmers, leading to low adoption and potentially slower technology evolution cycles. 
In an attempt generalize from existing architectures, ... we ... landscape ...''}
 the need for novel compiler technologies by presenting the landscape of CNM and CIM systems and highlighting the challenges associated with their programmability. 
Subsequently, it gives an overview of the CINM compiler, introducing its modules and backend targets.
\jc{The last sentence (content of this section) sounds a bit misplaced for me. If it already describes CINM, then I think it should be in the next section. If you want to have something similar here, then maybe you can place it as a vision of what is needed down the line (extensible, more backends, intelligent mapping onto het platforms, ...). Then you can say that CINM is an important step towards that vision. Does that make sense?}

% \jc{Depending on the taxonomy issue, this section could start with that. Given that the content here looks thin, this would really help}

\subsection{Programmability of CIM and CNM systems}
\label{subsec:motiv}
Fig.~\ref{fig:taxonomy} presents a partial taxonomy of the prominent and promising but less mature CNM and CIM systems. On the CNM side, the figure shows only real-world systems, leaving a multitude of previously proposed architectures. Similarly, only promising and mature CIM technologies are presented on the CIM side. 

\begin{figure}[tbh]
\includegraphics[width=\columnwidth]{figures/taxonomy.pdf}
\caption{A partial taxonomy of CNM and CIM systems based on pronounced technologies.}
\label{fig:taxonomy}
\end{figure}

\begin{figure}[tbh]
\includegraphics[width=\columnwidth]{figures/CINM_supported_ops.pdf}
\caption{CINM landscape. The figure shows the operations supported by various architectures and the granularities at which they can be re-programmed and retargetted.}
\label{fig:supp_ops}
\end{figure}


Unfortunately, even for this limited set of systems, programming models are
either nonexistent, or they can not be leveraged to program other systems.
These architectures are typically optimized for a specific domain or function
and use low-level, architecture-specific libraries to expose their device
traits. The radically different design decisions and overall architectures of
these systems make their programmability a serious challenge. For instance, in
UPMEM, the programmer is responsible for load balancing on thousands of DPUs,
explicit data movement between the CPUs and DPUs, MRAM and WRAM, and the data
coherency~\cite{UPMEM}. The AiM architecture has unique features that allow
operations including row clone, element-wise multiplication, and addition on a
set of banks with different granularities~\cite{skhynix}. However, it is not
clear how these systems are programmed. Samsung's FIMDRAM has its own
\emph{closed-source} software stack~\cite{samsungPIM}. The programming models
and tools of different CIM technologies, e.g., for PCM~\cite{occ}, do not apply
to other technologies (such as MRAM) as they have different device properties. 

Fig.~\ref{fig:soa-models} shows code examples of the GEMM\ak{or a smaller one}
kernel for various architectures. With their existing programming models, it is
next to impossible to program and effectively utilize heterogeneous systems
integrating these technologies. In addition, any device or system changes may
lead to a considerable rewriting of the input applications. To enable the
integration and exploration of these devices in heterogeneous setups, novel
programming models are needed that abstract from these devices to a higher
level that allows rigorous analysis and reasoning about individual kernels and
supports a richer set of optimizations and device interfaces. The next section
presents Cinnamon, our hierarchal compilation flow designed on these
principles.

% - Show a taxonomy of possible systems ~\\
% \jc{If a taxonomy exists that we can refer to, then this could stay here. If we come up with the taxonomy, this part should go somewhere else}
% - Code for UPMEM, CIM and other (tedious, hard to read examples)~\\
% - how should it look like for our infrastructure.
% \jc{Very good. An idea to make this more explicit would be to covey how much re-coding is needed if you decide to change something. Don't know what that could be, maybe a small expression rewrite, using a transposed matrix? The idea would be to show that at the DSL-level}

\begin{listing}[H]
\begin{minted}[breaklines, framesep=2mm, frame=lines, fontsize=\footnotesize]{c}
for(int i = 1; i < I - 1; i++)
  for(int j = 1; j < J - 1; j++)
R1:    lap[i][j] = in[i][j] + in[i+1][j] + in[i-1][j] + in[i][j+1] + in[i][j-1];
\end{minted}
\caption{Dummy code/placeholder for code}
\label{list:diffusion}
\end{listing}

\subsection{\cname lowering pipeline}
\label{subsec:overview}
Fig.~\ref{fig:flow} presents a high-level overview of the \cname compilation flow. \cname leverages MLIR and is designed in a modular way that can be easily extended to support other technologies. The entry point to the compiler is the \texttt{Linalg} dialect. Therefore, \cname can be used with any domain-specific language (DSL) or other high-level description of the computational kernel that can be lowered or raised to the \texttt{Linalg} dialect (see Sec.~\ref{subsec:frontend}). At the \texttt{Linalg} abstraction, \cname implements analysis passes to detect and rewrite computational motifs in a CINM-friendly representation. For instance, if so desired, these passes will rewrite convolutions and tensor contractions as matrix-matrix multiplication. The \texttt{Affine} dialect implements device-agnostic transformations, e.g., to improve locality and minimize memory accesses. The \texttt{Affine} dialect is then lowered to the \texttt{CINM} dialect that transparently decides the CNM or CIM class for the input kernel based on its computational and memory access patterns and lowers it to the respective \texttt{CIM} or \texttt{CNM} dialect. At both the \texttt{CIM} or \texttt{CNM} dialects, the analysis passes identify the potential hardware target based on the device properties. For instance, if the \texttt{CINM} analysis rout a GEMM kernel to the \texttt{CIM} dialect, the analysis at this abstraction decides whether to use the PCM or the RRAM target to accelerate it. The device-specific dialects then serve as interfaces to their respective accelerators and implement device-aware transformations. For instance, for UPMEM and FIMDRAM, these transformations maximize the WRAM and GRF localities, respectively, while for PCM/RRAM and RTM, these transformations reduce the number of writes and shifts, respectively. All device dialects are then lowered through the \texttt{SCF} and \texttt{Standard} dialects to the machine IR, mapping operations to their respective library calls or lowering them to the host CPU instructions.      

\begin{figure*}
\begin{center}
\includegraphics[scale=0.75]{./figures/SoftwareStack.pdf}
\caption{The Cinnamon compiler.}
\label{fig:flow}
\end{center}
\end{figure*}

